Predictable Accelerator Design with Time-Sensitive Affine Types

Field-programmable gate arrays (FPGAs) provide an opportunity to co-design applications with hardware accelerators, yet they remain difficult to program. High-level synthesis (HLS) tools promise to raise the level of abstraction by compiling C or C++ to accelerator designs. Repurposing legacy software languages, however, requires complex heuristics to map imperative code onto hardware structures. We find that the black-box heuristics in HLS can be unpredictable: changing parameters in the program that should improve performance can counterintuitively yield slower and larger designs. This paper proposes a type system that restricts HLS to programs that can predictably compile to hardware accelerators. The key idea is to model consumable hardware resources with a time-sensitive affine type system that prevents simultaneous uses of the same hardware structure. We implement the type system in Dahlia, a language that compiles to HLS C++, and show that it can reduce the size of HLS parameter spaces while accepting Pareto-optimal designs.

==> fig/Makefile <==
.PHONY: phony

EXP_FOLDER := ../../fuse-benchmarks-sdaccel/experiments
KEYS := lut-used runtime-avg
EXP_NAME := \
	gemm-no-part-unroll/no-partition-unrolling \
	gemm-const-unroll-part/const-unroll-partition \
	gemm-const-partition-unroll/const-partition-unroll \
	gemm-const-len-partition-and-unroll/const-len-partition-and-unroll

DSE := gemm-blocked-dse/gemm-blocked-dse
DSE_GRAPHS := only-dahlia only-pareto dahlia-pareto dahlia-non-pareto

SPATIAL_GRAPHS := \
	spatial-sweep/spatial-sweep-lut-used.pdf \
	spatial-sweep/paper-normalized.pdf

SOURCES := $(foreach X,$(EXP_NAME),$(foreach K,$(KEYS),$X-$K.pdf)) \
					 $(foreach D,$(DSE_GRAPHS),$(DSE)-$D.pdf) \
					 $(SPATIAL_GRAPHS)

$(SOURCES): phony
	$(MAKE) -C $(EXP_FOLDER) paper-experiments
	cp $(foreach S,$(SOURCES),$(EXP_FOLDER)/$S) ./

